Uncertainties of predictions from parton distribution functions II: the Hessian method

We develop a general method to quantify the uncertainties of parton distribution functions and their physical predictions, with emphasis on incorporating all relevant experimental constraints. The method uses the Hessian formalism to study an effective chi-squared function that quantifies the fit between theory and experiment. Key ingredients are a recently developed iterative procedure to calculate the Hessian matrix in the difficult global analysis environment, and the use of parameters defined as components along appropriately normalized eigenvectors. The result is a set of 2d Eigenvector Basis parton distributions (where d=16 is the number of parton parameters) from which the uncertainty on any physical quantity due to the uncertainty in parton distributions can be calculated. We illustrate the method by applying it to calculate uncertainties of gluon and quark distribution functions, W boson rapidity distributions, and the correlation between W and Z production cross sections.

==> pdf1.tbl0.tex <==
%%---LIST OF EXPERIMENTS---
\newcommand{\tblChiSq}
{
\begin{table}[htb]
\fontfamily{cmr}\fontsize{10}{10}\selectfont
\begin{center}
\begin{tabular}{|ccc||ccc|}
\hline
Current sets& $\chi^{2 \strut}$ & $\Delta \chi^{2}$
& Historical sets& $\chi^{2}$ & $ \Delta \chi^{2}$ \\
\hline
CTEQ5M1$^{\strut}$ & 1188 & - & CTEQ4M & 1540 & $352$ \\
CTEQ5HJ & 1272 & $84$ & MRSR2 & 1680 & $492$ \\
MRST99 & 1297 & $109$ & MRSR1 & 1758 & $570$ \\
MRST-$\alpha \downarrow $ & 1356 & $168$ & CTEQ3M & 2254 & $1066$ \\
MRST-$\alpha \uparrow $ & 1531 & $343$ & MRSA' & 3371 & $2183$ \\
\hline
\end{tabular}
\end{center}
\caption{
\fontfamily{cmr}\fontsize{12}{12}\selectfont
Overall $\chi_\mathrm{global}^2$ values and their increments above the
best fit value, for some current and historical parton distribution sets.
}
\label{tbl:ChiSq}
\end{table}
}


==> pdf1.tbl1.tex <==
%%---LIST OF EXPERIMENTS---
\newcommand{\tblDatSet}
{
\begin{table}[hbt]
\fontfamily{cmr}\fontsize{10}{10}\selectfont
\begin{center}
\begin{tabular}{|r|cr|cc|r|}
\hline
Expt $n$ & Process          & $N_n ^{\strut} \strut$ & Name & Ref. & $\Delta_n$ \\ \hline
1  & DIS $F_2(\mu p)^{\strut}$               & 168 & BCDMS & \cite{bcdms}   & $19.7$ \\
2  & DIS $F_2(\mu d)$                        & 156 & BCDMS & \cite{bcdms}   &  $4.5$ \\
3  & DIS $F_2(ep)$                           & 172 & H1    & \cite{NewH1}   &  $3.7$ \\
4  & DIS $F_2(ep)$                           & 186 & ZEUS  & \cite{NewZeus} &  $9.7$ \\
5  & DIS $F_2(\mu p)$                        & 104 & NMC   & \cite{NewNmc}  &  $7.8$ \\
6  & DIS $\mu p/\mu n$                       & 123 & NMC   & \cite{NewNmc}  &  $1.9$ \\
7  & DIS $\mu p/\mu n$                       &  13 & NMC   & \cite{NewNmc}  & $13.9$ \\
8  & DIS $F_2(\nu A)$                        &  87 & CCFR  & \cite{ccfr}    &  $8.9$ \\
9  & DIS $F_3(\nu A)$                        &  87 & CCFR  & \cite{ccfr}    &  $5.5$ \\
10 & D-Y $pp$                                & 119 & E605  & \cite{E605}    &  $6.4$ \\
11 & D-Y $pd/pp$                             &   1 & NA51  & \cite{NA51}    &  $0.5$ \\
12 & D-Y $pd/pp$                             &  11 & E866  & \cite{E866}    &  $0.6$ \\
13 & W$_{\mbox{lept. asym.}}$                &  11 & CDF   & \cite{Wasym}   & $15.1$ \\
14 & $\bar{p}p\rightarrow {\mathrm{jet}}\,X$ &  24 & D{\O} & \cite{D0Jets}  &  $3.4$ \\
15 & $\bar{p}p\rightarrow {\mathrm{jet}}\,X$ &  33 & CDF   & \cite{CdfJets} &  $3.7$ \\ \hline
\end{tabular}
\end{center}
\caption{
\fontfamily{cmr}\fontsize{12}{12}\selectfont
Data sets used in the global analysis.
If experiment $n$ is omitted,
$\Delta_n$ denotes the amount by which $\chi^2$
\emph{for the remaining 14 experiments} can be reduced
by readjusting the fit parameters.
\label{tbl:DatSet}
}
\end{table}
}


==> pdf1.tbl2.tex <==
%%---Extremes of A_i's, and the z_j's that produce them---
\newcommand{\tblAiMatrix}
{
\begin{table}[htb]
\fontfamily{cmr}\fontsize{9}{9}\selectfont
\begin{center}
\begin{tabular}{|cccrrrrrrrr|}
\hline
Parameter & Value & Error
& $\strut z_1$ & $z_2$  &$z_3$  &$z_4$  &$z_5$  &$z_6$  &$z_7$  &$z_8$ \\ & &
& $\strut z_9$ & $z_{10}$ & $z_{11}$ & $z_{12}$ & $z_{13}$ & $z_{14}$ & $z_{15}$ & $z_{16}$ \\
\hline
%A_1^uv = A_1^dv TruePar=21
$\strut^{\strut} A_1^{u_v} + 1$               & $0.466$       & $.094$
  & $  .04$ & $ -.01$ & $  .00$ & $ -.08$ & $ -.04$ & $ -.09$ & $  .05$ & $  .07$ \\ & &
  $ +   .083 \,  -.079$
  & $ -.06$ & $ -.06$ & $  .35$ & $ -.74$ & $ -.37$ & $ -.39$ & $ -.06$ & $  .00$ \\

%A_2^uv TruePar=15
$\strut^{\strut} A_2^{u_v}$                   & $3.360$       & $.122$
  & $ -.01$ & $ -.01$ & $  .03$ & $ -.14$ & $ -.07$ & $ -.37$ & $ -.32$ & $  .46$ \\ & &
  $ +   .112 \,  -.106$
  & $  .54$ & $ -.13$ & $  .06$ & $ -.23$ & $  .17$ & $  .09$ & $  .35$ & $  .04$ \\

%A_3^uv TruePar=16
$\strut^{\strut} \ln(1 + A_3^{u_v})$          & $2.553$       & $0.51$
  & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .06$ & $ -.01$ & $ -.06$ & $ -.07$ \\ & &
  $ +   .44 \,  -.45$
  & $  .10$ & $  .02$ & $ -.36$ & $  .73$ & $  .36$ & $  .41$ & $  .13$ & $  .03$ \\

%A_4^uv TruePar=17
$\strut^{\strut} A_4^{u_v}$                   & $0.855$       & $.118$
  & $  .01$ & $  .00$ & $ -.04$ & $  .19$ & $ -.09$ & $ -.13$ & $ -.29$ & $  .51$ \\ & &
  $ +   .110 \,  -.118$
  & $  .48$ & $ -.05$ & $  .05$ & $  .06$ & $  .47$ & $  .19$ & $  .30$ & $ -.01$ \\
\hline


%A_2^dv TruePar=18
$\strut^{\strut} A_2^{d_v}$                   & $4.230$       & $.45$
  & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .06$ & $ -.06$ & $  .00$ & $  .02$ \\ & &
  $ +   .45 \,  -.40$
  & $ -.05$ & $  .13$ & $  .72$ & $  .45$ & $  .32$ & $ -.23$ & $ -.30$ & $  .08$ \\

%A_3^dv TruePar=19
$\strut^{\strut} \ln(1 + A_3^{d_v})$          & $2.388$       & $0.64$
  & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $ -.04$ & $  .00$ & $  .04$ & $  .05$ \\ & &
  $ +   .59 \,  -.62$
  & $ -.08$ & $  .05$ & $ -.04$ & $  .88$ & $  .38$ & $  .26$ & $ -.03$ & $  .06$ \\

%A_4^dv TruePar=20
$\strut^{\strut} A_4^{d_v}$                   & $0.763$       & $0.30$
  & $  .00$ & $  .00$ & $  .00$ & $ -.01$ & $ -.06$ & $  .16$ & $ -.13$ & $ -.18$ \\ & &
  $ +   .24 \,   -.23$
  & $  .26$ & $  .11$ & $  .52$ & $  .37$ & $  .49$ & $ -.11$ & $ -.41$ & $  .08$ \\
\hline


%log(gluon momentum fraction) TruePar= 6
$\strut^{\strut} \ln {\widetilde{f_g}}^{\strut}$        & $-1.047$      & $.018$
  & $  .01$ & $  .79$ & $  .32$ & $  .12$ & $  .19$ & $ -.25$ & $ -.16$ & $  .09$ \\ & &
  $ +   .018 \,  -.019$
  & $ -.19$ & $  .26$ & $  .00$ & $ -.05$ & $ -.03$ & $  .00$ & $ -.06$ & $ -.11$ \\

% A_1^g (+1) TruePar= 2
$\strut^{\strut} A_1^{g} + 1$                 & $0.469$       & $0.40$
  & $  .00$ & $  .00$ & $  .02$ & $  .01$ & $  .02$ & $  .02$ & $  .23$ & $  .05$ \\ & &
  $ +   0.39 \,  -0.35$
  & $  .22$ & $  .29$ & $  .00$ & $  .03$ & $ -.09$ & $  .04$ & $  .12$ & $  .89$ \\

%A_2^g TruePar= 3
$\strut^{\strut} A_2^{g}$                     & $5.574$       & $2.65$
  & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .00$ \\ & &
  $ +   2.98 \,  -2.30$
  & $  .00$ & $ -.03$ & $  .01$ & $  .01$ & $ -.03$ & $  .03$ & $  .11$ & $  .99$ \\
\hline


%A_1^(ubar+dbar) TruePar= 7
$\strut^{\strut} A_1^{\bar{d}+\bar{u} \strut} + 1$   & $-.009$      & $.148$
  & $  .00$ & $ -.03$ & $  .10$ & $  .07$ & $  .01$ & $  .01$ & $ -.24$ & $ -.07$ \\ & &
  $ +   .142  \,  -.119$
  & $ -.15$ & $ -.65$ & $  .06$ & $  .15$ & $ -.13$ & $ -.07$ & $ -.09$ & $ -.65$ \\


%A_2^(ubar+dbar) TruePar= 8
$\strut^{\strut} A_2^{\bar{d}+\bar{u}}$       & $7.866$       & $0.96$
  & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .04$ & $  .00$ \\ & &
  $ +   1.05  \,  -1.09$
  & $  .01$ & $ -.21$ & $  .03$ & $ -.15$ & $  .89$ & $  .28$ & $ -.10$ & $ -.22$ \\

%A_3^(ubar+dbar) TruePar= 9
$\strut^{\strut} \ln(1+A_3^{\bar{d}+\bar{u}})$ & $2.031$       & $0.89$
  & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $ -.03$ & $  .00$ \\ & &
  $ +   .78  \,  -.89$
  & $ -.04$ & $  .29$ & $ -.05$ & $ -.28$ & $  .66$ & $  .20$ & $  .04$ & $  .59$ \\
\hline


%log(B_0) TruePar=10
$\strut^{\strut} \ln B_0^{\bar{d}/\bar{u} \strut}$   & $10.29$      & $1.45$
  & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $ -.01$ & $ -.02$ & $  .01$ & $ -.04$ \\ & &
  $ +   1.551  \,  -1.496$
  & $  .00$ & $  .01$ & $  .03$ & $  .00$ & $  .00$ & $  .06$ & $  .94$ & $ -.32$ \\

%B_1 TruePar=11
$\strut^{\strut} B_1^{\bar{d}/\bar{u}}$       & $5.379$       & $0.85$
  & $  .00$ & $  .00$ & $  .00$ & $ -.01$ & $  .02$ & $  .06$ & $ -.02$ & $  .10$ \\ & &
  $ +   1.02   \, -.75$
  & $ -.02$ & $ -.03$ & $  .01$ & $  .04$ & $  .16$ & $ -.21$ & $  .93$ & $ -.24$ \\

%B_4 TruePar=14
$\strut^{\strut} B_4^{\bar{d}/\bar{u}}$       & $4.498$       & $1.21$
  & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .00$ & $  .01$ & $  .00$ & $  .01$ \\ & &
  $ +   1.20  \,  -1.12$
  & $  .00$ & $  .01$ & $  .06$ & $ -.04$ & $ -.27$ & $  .94$ & $ -.01$ & $ -.20$ \\
\hline
\hline
\end{tabular}
\end{center}
\caption{
\fontfamily{cmr}\fontsize{12}{12}\selectfont
Parameters of the global fit.  Errors shown are for $T \! = \! 5$,
{\textit i.e.}, $\Delta \chi_{\rm global}^2 = 25$.
Fixed parameters:
$A_4^{\bar{d}+\bar{u}} \! = \! 1.0$,
$B_2^{\bar{d}/\bar{u}} \! = \! 15.0$,
$B_3^{\bar{d}/\bar{u}} \! = \! 10.0$, and
$A_3^{g} \! = \! 0.0 \, \Rightarrow \, A_4^{g} \, {\rm irrelevant}$.
The $z_k$ are proportional to the
$z_k(a_{i}^{\pm }) = \pm \, t \, M_{ik}$ of Eq.~(\ref{eq:zsubi})
and are normalized to $\sum_k z_k^{2} = 1$.
\label{tbl:AiMatrix}
}
\end{table}
}


==> pdf1.tbl3.tex <==
%%---Parameters for Best Fit and up/dn sets 1-8 --
\newcommand{\tblUpDnA}
{
\begin{table}[htb]
\fontfamily{cmr}\fontsize{9}{9}\selectfont
\begin{center}
\begin{tabular}{|rrrrr|rrrrr|}
 \hline
 \hline
 % (npar=16 chisqr min=   1188.75     up/down sets DChisqr=   25.00 setau101.up4
 %Chisqr minimum set:
 $ -0.1941$ & $ -0.5337$ & $  3.3604$ & $ 11.8404$ & $  0.8552$ &
 $\strut^{\strut}_{\strut} \ln A_0^{u_v}$ &
 $A_1^{u_v}$ &
 $A_2^{u_v}$ &
 $A_3^{u_v}$ &
 $A_4^{u_v}$ \\
 $ -0.7175$ & $ -0.5337$ & $  4.2296$ & $  9.8950$ & $  0.7628$ &
 $\strut^{\strut}_{\strut} \ln A_0^{d_v}$ &
 $A_1^{d_v}$ &
 $A_2^{d_v}$ &
 $A_3^{d_v}$ &
 $A_4^{d_v}$ \\
 $  1.8914$ & $ -0.5305$ & $  5.5737$ & $  0.0000$ & $  1.0000$ &
 $\strut^{\strut}_{\strut} \ln A_0^{g}$ &
 $A_1^{g}$ &
 $A_2^{g}$ &
 $A_3^{g}$ &
 $A_4^{g}$ \\
 $ -1.1174$ & $ -1.0092$ & $  7.8658$ & $  6.6187$ & $  1.0000$ &
 $\strut^{\strut}_{\strut} \ln A_0^{\bar{d} + \bar{u}}$ &
 $A_1^{\bar{d} + \bar{u}}$ &
 $A_2^{\bar{d} + \bar{u}}$ &
 $A_3^{\bar{d} + \bar{u}}$ &
 $A_4^{\bar{d} + \bar{u}}$ \\
 $ 10.2940$ & $  5.3793$ & $ 15.0000$ & $ 10.0000$ & $  4.4980$ &
 $\strut^{\strut}_{\strut} \ln B_0^{\bar{d} / \bar{u}}$ &
 $B_1^{\bar{d} / \bar{u}}$ &
 $B_2^{\bar{d} / \bar{u}}$ &
 $B_3^{\bar{d} / \bar{u}}$ &
 $B_4^{\bar{d} / \bar{u}}$ \\
 \hline
 \hline
 $\strut^{\strut}$
 %ipar= 1
 $ -0.1841$ & $ -0.5298$ & $  3.3596$ & $ 11.8478$ & $  0.8558$ &
 $ -0.2042$ & $ -0.5376$ & $  3.3612$ & $ 11.8331$ & $  0.8546$ \\
 $ -0.7064$ & $ -0.5298$ & $  4.2295$ & $  9.8957$ & $  0.7629$ &
 $ -0.7285$ & $ -0.5376$ & $  4.2297$ & $  9.8942$ & $  0.7627$ \\
 $  1.8919$ & $ -0.5304$ & $  5.5737$ & $  0.0000$ & $  1.0000$ &
 $  1.8910$ & $ -0.5306$ & $  5.5737$ & $  0.0000$ & $  1.0000$ \\
 $ -1.1342$ & $ -1.0089$ & $  7.8658$ & $  6.6191$ & $  1.0000$ &
 $ -1.1010$ & $ -1.0095$ & $  7.8658$ & $  6.6182$ & $  1.0000$ \\
 $ 10.2940$ & $  5.3793$ & $ 15.0000$ & $ 10.0000$ & $  4.4980$ &
 $ 10.2940$ & $  5.3793$ & $ 15.0000$ & $ 10.0000$ & $  4.4980$ \\
 %number sum rules: up= 2.00001 dn= 1.00001 | up= 2.00002 dn= 1.00001
 %momentum sum rule: 0.999996 | 0.999996
 \hline
 $\strut^{\strut}$
 %ipar= 2
 $ -0.1951$ & $ -0.5343$ & $  3.3597$ & $ 11.8372$ & $  0.8557$ &
 $ -0.1931$ & $ -0.5331$ & $  3.3611$ & $ 11.8437$ & $  0.8547$ \\
 $ -0.7184$ & $ -0.5343$ & $  4.2291$ & $  9.8952$ & $  0.7636$ &
 $ -0.7165$ & $ -0.5331$ & $  4.2301$ & $  9.8947$ & $  0.7620$ \\
 $  1.9025$ & $ -0.5321$ & $  5.5740$ & $  0.0000$ & $  1.0000$ &
 $  1.8802$ & $ -0.5288$ & $  5.5734$ & $  0.0000$ & $  1.0000$ \\
 $ -1.1609$ & $ -1.0140$ & $  7.8662$ & $  6.6117$ & $  1.0000$ &
 $ -1.0751$ & $ -1.0043$ & $  7.8654$ & $  6.6256$ & $  1.0000$ \\
 $ 10.2940$ & $  5.3794$ & $ 15.0000$ & $ 10.0000$ & $  4.4980$ &
 $ 10.2940$ & $  5.3792$ & $ 15.0000$ & $ 10.0000$ & $  4.4980$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00001 dn= 1.00001
 %momentum sum rule: 0.999996 | 0.999995
 \hline
 $\strut^{\strut}$
 %ipar= 3
 $ -0.1981$ & $ -0.5338$ & $  3.3645$ & $ 11.8237$ & $  0.8501$ &
 $ -0.1903$ & $ -0.5336$ & $  3.3564$ & $ 11.8567$ & $  0.8602$ \\
 $ -0.7182$ & $ -0.5338$ & $  4.2287$ & $  9.9098$ & $  0.7633$ &
 $ -0.7167$ & $ -0.5336$ & $  4.2304$ & $  9.8806$ & $  0.7623$ \\
 $  1.9095$ & $ -0.5244$ & $  5.5730$ & $  0.0000$ & $  1.0000$ &
 $  1.8738$ & $ -0.5364$ & $  5.5745$ & $  0.0000$ & $  1.0000$ \\
 $ -1.0925$ & $ -0.9946$ & $  7.8651$ & $  6.6340$ & $  1.0000$ &
 $ -1.1422$ & $ -1.0234$ & $  7.8665$ & $  6.6037$ & $  1.0000$ \\
 $ 10.2939$ & $  5.3795$ & $ 15.0000$ & $ 10.0000$ & $  4.4980$ &
 $ 10.2941$ & $  5.3791$ & $ 15.0000$ & $ 10.0000$ & $  4.4980$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00002 dn= 1.00001
 %momentum sum rule: 0.999996 | 0.999996
 \hline
 $\strut^{\strut}$
 %ipar= 4
 $ -0.1932$ & $ -0.5413$ & $  3.3436$ & $ 11.8275$ & $  0.8774$ &
 $ -0.1960$ & $ -0.5260$ & $  3.3774$ & $ 11.8536$ & $  0.8327$ \\
 $ -0.7420$ & $ -0.5413$ & $  4.2312$ & $  9.8814$ & $  0.7592$ &
 $ -0.6928$ & $ -0.5260$ & $  4.2279$ & $  9.9087$ & $  0.7664$ \\
 $  1.9005$ & $ -0.5271$ & $  5.5735$ & $  0.0000$ & $  1.0000$ &
 $  1.8822$ & $ -0.5340$ & $  5.5739$ & $  0.0000$ & $  1.0000$ \\
 $ -1.0798$ & $ -0.9990$ & $  7.8655$ & $  6.6250$ & $  1.0000$ &
 $ -1.1544$ & $ -1.0195$ & $  7.8661$ & $  6.6122$ & $  1.0000$ \\
 $ 10.2964$ & $  5.3748$ & $ 15.0000$ & $ 10.0000$ & $  4.4970$ &
 $ 10.2916$ & $  5.3839$ & $ 15.0000$ & $ 10.0000$ & $  4.4990$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00001 dn= 1.00001
 %momentum sum rule: 0.999995 | 0.999995
 \hline
 $\strut^{\strut}$
 %ipar= 5
 $ -0.2373$ & $ -0.5372$ & $  3.3513$ & $ 12.2488$ & $  0.8440$ &
 $ -0.1528$ & $ -0.5303$ & $  3.3692$ & $ 11.4555$ & $  0.8661$ \\
 $ -0.7278$ & $ -0.5372$ & $  4.2550$ & $  9.5924$ & $  0.7435$ &
 $ -0.7078$ & $ -0.5303$ & $  4.2049$ & $ 10.1974$ & $  0.7816$ \\
 $  1.9071$ & $ -0.5244$ & $  5.5733$ & $  0.0000$ & $  1.0000$ &
 $  1.8761$ & $ -0.5364$ & $  5.5742$ & $  0.0000$ & $  1.0000$ \\
 $ -1.1096$ & $ -1.0071$ & $  7.8668$ & $  6.6099$ & $  1.0000$ &
 $ -1.1246$ & $ -1.0112$ & $  7.8648$ & $  6.6272$ & $  1.0000$ \\
 $ 10.2848$ & $  5.3943$ & $ 15.0000$ & $ 10.0000$ & $  4.5012$ &
 $ 10.3029$ & $  5.3647$ & $ 15.0000$ & $ 10.0000$ & $  4.4949$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00002 dn= 1.00001
 %momentum sum rule: 0.999996 | 0.999996
 \hline
 $\strut^{\strut}$
 %ipar= 6
 $ -0.2370$ & $ -0.5419$ & $  3.3147$ & $ 11.7529$ & $  0.8399$ &
 $ -0.1529$ & $ -0.5258$ & $  3.4046$ & $ 11.9257$ & $  0.8700$ \\
 $ -0.6899$ & $ -0.5419$ & $  4.2039$ & $  9.8658$ & $  0.8113$ &
 $ -0.7483$ & $ -0.5258$ & $  4.2545$ & $  9.9232$ & $  0.7159$ \\
 $  1.9021$ & $ -0.5228$ & $  5.5734$ & $  0.0000$ & $  1.0000$ &
 $  1.8811$ & $ -0.5379$ & $  5.5741$ & $  0.0000$ & $  1.0000$ \\
 $ -1.0919$ & $ -1.0074$ & $  7.8633$ & $  6.6099$ & $  1.0000$ &
 $ -1.1398$ & $ -1.0109$ & $  7.8682$ & $  6.6271$ & $  1.0000$ \\
 $ 10.2670$ & $  5.4325$ & $ 15.0000$ & $ 10.0000$ & $  4.5101$ &
 $ 10.3201$ & $  5.3279$ & $ 15.0000$ & $ 10.0000$ & $  4.4863$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00002 dn= 1.00001
 %momentum sum rule: 0.999996 | 0.999996
 \hline
 $\strut^{\strut}$
 %ipar= 7
 $ -0.2078$ & $ -0.5282$ & $  3.3181$ & $ 11.4087$ & $  0.8179$ &
 $ -0.1833$ & $ -0.5383$ & $  3.3960$ & $ 12.2156$ & $  0.8866$ \\
 $ -0.7700$ & $ -0.5282$ & $  4.2279$ & $ 10.1816$ & $  0.7198$ &
 $ -0.6769$ & $ -0.5383$ & $  4.2310$ & $  9.6594$ & $  0.7990$ \\
 $  2.0853$ & $ -0.4301$ & $  5.5687$ & $  0.0000$ & $  1.0000$ &
 $  1.7217$ & $ -0.6150$ & $  5.5779$ & $  0.0000$ & $  1.0000$ \\
 $ -1.2032$ & $ -1.0484$ & $  7.9025$ & $  6.3721$ & $  1.0000$ &
 $ -1.0446$ & $ -0.9762$ & $  7.8349$ & $  6.8326$ & $  1.0000$ \\
 $ 10.3046$ & $  5.3626$ & $ 15.0000$ & $ 10.0000$ & $  4.4919$ &
 $ 10.2850$ & $  5.3934$ & $ 15.0000$ & $ 10.0000$ & $  4.5031$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00002 dn= 1.00001
 %momentum sum rule: 0.999996 | 0.999996
 \hline
 $\strut^{\strut}$
 %ipar= 8
 $ -0.0801$ & $ -0.5269$ & $  3.4174$ & $ 11.3977$ & $  0.9160$ &
 $ -0.3093$ & $ -0.5402$ & $  3.3060$ & $ 12.2779$ & $  0.7971$ \\
 $ -0.7805$ & $ -0.5269$ & $  4.2376$ & $ 10.2241$ & $  0.7090$ &
 $ -0.6640$ & $ -0.5402$ & $  4.2220$ & $  9.5897$ & $  0.8142$ \\
 $  1.9359$ & $ -0.5086$ & $  5.5686$ & $  0.0000$ & $  1.0000$ &
 $  1.8485$ & $ -0.5514$ & $  5.5786$ & $  0.0000$ & $  1.0000$ \\
 $ -1.1401$ & $ -1.0195$ & $  7.8611$ & $  6.6228$ & $  1.0000$ &
 $ -1.0838$ & $ -0.9994$ & $  7.8703$ & $  6.6147$ & $  1.0000$ \\
 $ 10.2407$ & $  5.4629$ & $ 15.0000$ & $ 10.0000$ & $  4.5154$ &
 $ 10.3449$ & $  5.2995$ & $ 15.0000$ & $ 10.0000$ & $  4.4814$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00002 dn= 1.00001
 %momentum sum rule: 0.999996 | 0.999994
 \hline
\end{tabular}
\end{center}
\caption{
\fontfamily{cmr}\fontsize{12}{12}\selectfont
Parameters of the Best Fit $S_0$ and their definitions, followed by
Eigenvector Sets $S_1^+, S_1^-, S_2^+, S_2^-, \dots$.
\label{tbl:UpDnA}
}
\end{table}
}


==> pdf1.tbl4.tex <==
%%---Parameters for up/dn sets 8-16 --
\newcommand{\tblUpDnB}
{
\begin{table}[htb]
\fontfamily{cmr}\fontsize{9}{9}\selectfont
\begin{center}
\begin{tabular}{|rrrrr|rrrrr|}
 \hline
 $\strut^{\strut}$
 %ipar= 9
 $ -0.1659$ & $ -0.5391$ & $  3.4265$ & $ 12.5012$ & $  0.9121$ &
 $ -0.2243$ & $ -0.5283$ & $  3.2943$ & $ 11.2121$ & $  0.7983$ \\
 $ -0.6220$ & $ -0.5391$ & $  4.2087$ & $  9.3472$ & $  0.8414$ &
 $ -0.8285$ & $ -0.5283$ & $  4.2505$ & $ 10.4716$ & $  0.6842$ \\
 $  2.0550$ & $ -0.4456$ & $  5.5690$ & $  0.0000$ & $  1.0000$ &
 $  1.7218$ & $ -0.6154$ & $  5.5785$ & $  0.0000$ & $  1.0000$ \\
 $ -1.1277$ & $ -1.0312$ & $  7.8798$ & $  6.3693$ & $  1.0000$ &
 $ -1.0969$ & $ -0.9873$ & $  7.8518$ & $  6.8764$ & $  1.0000$ \\
 $ 10.2997$ & $  5.3659$ & $ 15.0000$ & $ 10.0000$ & $  4.4929$ &
 $ 10.2883$ & $  5.3927$ & $ 15.0000$ & $ 10.0000$ & $  4.5031$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00002 dn= 1.00001
 %momentum sum rule: 0.999996 | 0.999996
 \hline
 $\strut^{\strut}$
 %ipar=10
 $ -0.2209$ & $ -0.5385$ & $  3.3464$ & $ 11.9679$ & $  0.8505$ &
 $ -0.1581$ & $ -0.5272$ & $  3.3793$ & $ 11.6700$ & $  0.8616$ \\
 $ -0.7087$ & $ -0.5385$ & $  4.2773$ & $ 10.1973$ & $  0.7903$ &
 $ -0.7304$ & $ -0.5272$ & $  4.1650$ & $  9.4988$ & $  0.7256$ \\
 $  2.0697$ & $ -0.4336$ & $  5.4996$ & $  0.0000$ & $  1.0000$ &
 $  1.6342$ & $ -0.6616$ & $  5.6741$ & $  0.0000$ & $  1.0000$ \\
 $ -1.4530$ & $ -1.0911$ & $  7.6927$ & $  8.5071$ & $  1.0000$ &
 $ -0.6805$ & $ -0.8983$ & $  8.1000$ & $  4.6459$ & $  1.0000$ \\
 $ 10.3080$ & $  5.3568$ & $ 15.0000$ & $ 10.0000$ & $  4.5032$ &
 $ 10.2750$ & $  5.4097$ & $ 15.0000$ & $ 10.0000$ & $  4.4910$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00002 dn= 1.00001
 %momentum sum rule: 0.999996 | 0.999997
 \hline
 $\strut^{\strut}$
 %ipar=11
 $  0.0212$ & $ -0.4998$ & $  3.3685$ & $  9.5867$ & $  0.8619$ &
 $ -0.3963$ & $ -0.5645$ & $  3.3530$ & $ 14.3021$ & $  0.8491$ \\
 $ -0.3803$ & $ -0.4998$ & $  4.5680$ & $  9.5749$ & $  0.9267$ &
 $ -1.0637$ & $ -0.5645$ & $  3.9221$ & $ 10.1942$ & $  0.6138$ \\
 $  1.8986$ & $ -0.5295$ & $  5.5981$ & $  0.0000$ & $  1.0000$ &
 $  1.8849$ & $ -0.5314$ & $  5.5516$ & $  0.0000$ & $  1.0000$ \\
 $ -1.0511$ & $ -0.9997$ & $  7.8935$ & $  6.2437$ & $  1.0000$ &
 $ -1.1519$ & $ -1.0178$ & $  7.8406$ & $  6.9762$ & $  1.0000$ \\
 $ 10.3431$ & $  5.3894$ & $ 15.0000$ & $ 10.0000$ & $  4.5718$ &
 $ 10.2494$ & $  5.3702$ & $ 15.0000$ & $ 10.0000$ & $  4.4309$ \\
 %number sum rules: up= 2.00001 dn= 1.00001 | up= 2.00002 dn= 0.99999
 %momentum sum rule: 0.999996 | 0.999996
 \hline
 $\strut^{\strut}$
 %ipar=12
 $ -0.6200$ & $ -0.6029$ & $  3.3322$ & $ 17.6542$ & $  0.8617$ &
 $  0.2128$ & $ -0.4640$ & $  3.3889$ & $  7.8121$ & $  0.8487$ \\
 $ -1.0990$ & $ -0.6029$ & $  4.4299$ & $ 18.0058$ & $  0.8742$ &
 $ -0.3418$ & $ -0.4640$ & $  4.0277$ & $  5.2176$ & $  0.6505$ \\
 $  1.9215$ & $ -0.5171$ & $  5.5927$ & $  0.0000$ & $  1.0000$ &
 $  1.8610$ & $ -0.5440$ & $  5.5546$ & $  0.0000$ & $  1.0000$ \\
 $ -0.9608$ & $ -0.9876$ & $  7.7202$ & $  4.9575$ & $  1.0000$ &
 $ -1.2706$ & $ -1.0310$ & $  8.0126$ & $  8.7623$ & $  1.0000$ \\
 $ 10.2885$ & $  5.4121$ & $ 15.0000$ & $ 10.0000$ & $  4.4446$ &
 $ 10.2995$ & $  5.3462$ & $ 15.0000$ & $ 10.0000$ & $  4.5518$ \\
 %number sum rules: up= 2.00003 dn= 1.00002 | up= 2.00001 dn= 1.00001
 %momentum sum rule: 0.999995 | 0.999996
 \hline
 $\strut^{\strut}$
 %ipar=13
 $ -0.3285$ & $ -0.5667$ & $  3.3800$ & $ 14.2366$ & $  0.9075$ &
 $ -0.0441$ & $ -0.4965$ & $  3.3383$ & $  9.5883$ & $  0.7962$ \\
 $ -0.7740$ & $ -0.5667$ & $  4.3664$ & $ 12.6923$ & $  0.9007$ &
 $ -0.6624$ & $ -0.4965$ & $  4.0754$ & $  7.4209$ & $  0.6073$ \\
 $  1.8124$ & $ -0.5621$ & $  5.5060$ & $  0.0000$ & $  1.0000$ &
 $  1.9800$ & $ -0.4949$ & $  5.6501$ & $  0.0000$ & $  1.0000$ \\
 $ -1.3022$ & $ -1.0266$ & $  8.6732$ & $ 12.2662$ & $  1.0000$ &
 $ -0.9707$ & $ -0.9896$ & $  6.9557$ & $  3.0774$ & $  1.0000$ \\
 $ 10.2946$ & $  5.5039$ & $ 15.0000$ & $ 10.0000$ & $  4.1962$ &
 $ 10.2934$ & $  5.2389$ & $ 15.0000$ & $ 10.0000$ & $  4.8382$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00001 dn= 1.00001
 %momentum sum rule: 0.999995 | 0.999996
 \hline
 $\strut^{\strut}$
 %ipar=14
 $ -0.4030$ & $ -0.5716$ & $  3.3718$ & $ 14.9177$ & $  0.8788$ &
 $ -0.0012$ & $ -0.4980$ & $  3.3497$ & $  9.4869$ & $  0.8330$ \\
 $ -0.9934$ & $ -0.5716$ & $  4.1229$ & $ 11.9127$ & $  0.7280$ &
 $ -0.4696$ & $ -0.4980$ & $  4.3301$ & $  8.2828$ & $  0.7956$ \\
 $  1.9461$ & $ -0.5128$ & $  5.6623$ & $  0.0000$ & $  1.0000$ &
 $  1.8398$ & $ -0.5471$ & $  5.4902$ & $  0.0000$ & $  1.0000$ \\
 $ -1.1804$ & $ -1.0206$ & $  8.1430$ & $  8.1232$ & $  1.0000$ &
 $ -1.0571$ & $ -0.9985$ & $  7.6046$ & $  5.4285$ & $  1.0000$ \\
 $ 10.3763$ & $  5.1976$ & $ 15.0000$ & $ 10.0000$ & $  5.6698$ &
 $ 10.2164$ & $  5.5506$ & $ 15.0000$ & $ 10.0000$ & $  3.3936$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00001 dn= 1.00001
 %momentum sum rule: 0.999995 | 0.999995
 \hline
 $\strut^{\strut}$
 %ipar=15
 $ -0.2036$ & $ -0.5399$ & $  3.4062$ & $ 12.7490$ & $  0.8931$ &
 $ -0.1860$ & $ -0.5282$ & $  3.3199$ & $ 11.0884$ & $  0.8217$ \\
 $ -0.9051$ & $ -0.5399$ & $  4.0867$ & $  9.6572$ & $  0.6340$ &
 $ -0.5709$ & $ -0.5282$ & $  4.3557$ & $ 10.1093$ & $  0.8765$ \\
 $  2.0530$ & $ -0.4819$ & $  5.8758$ & $  0.0000$ & $  1.0000$ &
 $  1.7480$ & $ -0.5734$ & $  5.3071$ & $  0.0000$ & $  1.0000$ \\
 $ -1.1784$ & $ -1.0238$ & $  7.7670$ & $  6.9327$ & $  1.0000$ &
 $ -1.0517$ & $ -0.9963$ & $  7.9530$ & $  6.3518$ & $  1.0000$ \\
 $ 11.7435$ & $  6.2127$ & $ 15.0000$ & $ 10.0000$ & $  4.4913$ &
 $  9.0144$ & $  4.6435$ & $ 15.0000$ & $ 10.0000$ & $  4.5039$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00002 dn= 1.00001
 %momentum sum rule: 0.999996 | 0.999996
 \hline
 $\strut^{\strut}$
 %ipar=16
 $ -0.2054$ & $ -0.5338$ & $  3.3661$ & $ 12.0453$ & $  0.8534$ &
 $ -0.1853$ & $ -0.5336$ & $  3.3560$ & $ 11.6819$ & $  0.8566$ \\
 $ -0.7110$ & $ -0.5338$ & $  4.2688$ & $ 10.4095$ & $  0.7879$ &
 $ -0.7226$ & $ -0.5336$ & $  4.1988$ & $  9.5075$ & $  0.7431$ \\
 $  3.2798$ & $ -0.1380$ & $  8.5257$ & $  0.0000$ & $  1.0000$ &
 $  0.7313$ & $ -0.8385$ & $  3.2571$ & $  0.0000$ & $  1.0000$ \\
 $ -1.7279$ & $ -1.1163$ & $  7.6289$ & $ 12.7489$ & $  1.0000$ &
 $ -0.6889$ & $ -0.9252$ & $  8.0517$ & $  3.7937$ & $  1.0000$ \\
 $  9.7697$ & $  5.1479$ & $ 15.0000$ & $ 10.0000$ & $  4.2287$ &
 $ 10.7054$ & $  5.5609$ & $ 15.0000$ & $ 10.0000$ & $  4.7094$ \\
 %number sum rules: up= 2.00002 dn= 1.00001 | up= 2.00002 dn= 1.00001
 %momentum sum rule: 0.999996 | 0.999996
 \hline
 \hline
\end{tabular}
\end{center}
\caption{
\fontfamily{cmr}\fontsize{12}{12}\selectfont
Continuation of Table \ref{tbl:UpDnA}: parameters of the Eigenvector
Sets $S_9^+, S_9^-$, \dots, $S_{16}^+, S_{16}^-$.
\label{tbl:UpDnB}
}
\end{table}
}

